Exploring Quantum Bootstrap Sampling for AQP Error Assessment: A Pilot Study

Error assessment for Approximate Query Processing (AQP) is a challenging problem. Bootstrap sampling can produce error assessment even when the population data distribution is unknown. However, bootstrap sampling needs to produce a large number of resamples with replacement, which is a computationally intensive procedure. In this paper, we introduce a quantum bootstrap sampling (QBS) framework to generate bootstrap samples on a quantum computer and produce an error assessment for AQP query estimations. The quantum circuit design is included in this framework.

==> template/markdown-header.tex <==

%% reference: https://mirror.mwt.me/ctan/macros/generic/markdown/markdown.html

\usepackage[footnotes,citations,inlineFootnotes,definitionLists,
hashEnumerators,smartEllipses,html,
fencedCode,hybrid,pipeTables,tableCaptions,
%texComments,strikeThrough,taskLists,rawAttribute,
underscores=false]{markdown}

%%---work around lncs package---
\makeatletter
\newcommand{\@chapapp}{\relax}%
\makeatother

%%---make markdown table not to float top---
\usepackage{float}
\makeatletter
\renewcommand*{\fps@table}{H}
\makeatother

%%---setup caption floating position---
%need package caption and float
% \usepackage{float}
\usepackage[skip=0.1\baselineskip]{caption} % space between caption and table be smaller

%%----set caption below----
%% https://github.com/Witiko/markdown/issues/32
%% https://github.com/Witiko/markdown/blob/31d90e65a97bccef616a81b33b46b417e212cdd7/markdown.dtx#L27540-L27623
%%
% \floatstyle{plain}  % Setup float package to always put captions below tables
% \restylefloat{table}
% \captionsetup[table]{position=below}  % Setup caption package to place \abovetopsep between caption and table

%%----set caption above---
\floatstyle{plaintop}  % Setup float package to always put captions above tables
\restylefloat{table}
\captionsetup[table]{position=above}  % Setup caption package to place \abovetopsep between caption and table

%% example: ![caption\label{fig1}](file_path "0.x") e.g. 0.8 means 0.8\linewidth
\markdownSetup{renderers={
    image = {\begin{figure}[hbt!]
        \centering
        \ifx&#4&
        \includegraphics[width=0.5\linewidth]{#3} %%default 0.5\linewidth
        %\includegraphics[scale=0.5]{#3} %%default 0.5\linewidth
        \else
        \includegraphics[width=#4\linewidth]{#3}
        %\includegraphics[scale=#4]{#3}
        \fi  
        \ifx&#1&\else
        \caption{#1}%
        \fi
        \end{figure}},
    link = {\href{#2}{#1}},
    %  headingThree = {\begin{frame}\frametitle{#1}},
    %  headingFour = {\begin{block}{#1}},
    %  horizontalRule = {\end{block}}
}}

% \markdownSetup{rendererPrototypes={
%   table = {%
%     \markdownLaTeXTable={}%
%     \markdownLaTeXTableAlignment={}%
%     \markdownLaTeXTableEnd={%
%       \markdownLaTeXBottomRule
%       \end{tabular}}%
%     \ifx\empty#1\empty\else
%       \addto@hook\markdownLaTeXTable{%
%         \begin{table}
%         \centering}%
%       \addto@hook\markdownLaTeXTableEnd{%
%         \caption{#1}
%         \end{table}}%
%     \fi
%     \addto@hook\markdownLaTeXTable{\begin{tabular}}%
%     \markdownLaTeXRowCounter=0%
%     \markdownLaTeXRowTotal=#2%
%     \markdownLaTeXColumnTotal=#3%
%     \markdownLaTeXRenderTableRow
%   }
% }}




